DBAT: Dynamic Backward Attention Transformer for Material Segmentation with Cross-Resolution Patches

The objective of dense material segmentation is to identify the material categories for every image pixel. Recent studies adopt image patches to extract material features. Although the trained networks can improve the segmentation performance, their methods choose a fixed patch resolution which fails to take into account the variation in pixel area covered by each material. In this paper, we propose the Dynamic Backward Attention Transformer (DBAT) to aggregate cross-resolution features. The DBAT takes cropped image patches as input and gradually increases the patch resolution by merging adjacent patches at each transformer stage, instead of fixing the patch resolution during training. We explicitly gather the intermediate features extracted from cross-resolution patches and merge them dynamically with predicted attention masks. Experiments show that our DBAT achieves an accuracy of 86.85%, which is the best performance among state-of-the-art real-time models. Like other successful deep learning solutions with complex architectures, the DBAT also suffers from lack of interpretability. To address this problem, this paper examines the properties that the DBAT makes use of. By analysing the cross-resolution features and the attention weights, this paper interprets how the DBAT learns from image patches. We further align features to semantic labels, performing network dissection, to infer that the proposed model can extract material-related features better than other methods. We show that the DBAT model is more robust to network initialisation, and yields fewer variable predictions compared to other models. The project code is available at https://github.com/heng-yuwen/Dynamic-Backward-Attention-Transformer.

==> modules/7.application.tex <==
\section{Application}
This section briefly introduces a specific application, visual-based room acoustic modelling \cite{mona2022audio}, that relies on our DBAT to provide the segmented materials for a specific room image taken by a 360$^{\circ}$  camera. The overall system is shown in Fig. \ref{3d_scenes_mat}. When predicting the material labels for the equal-rectangular projected 360$^{\circ}$ image, it is first projected into six cubes \cite{li2017projection} to cope with the panoramic distortion. Then the segmented images for the cubes are stitched back so that each pixel of the 360$^{\circ}$ image has one corresponding material label. Then the 3D scene is constructed with the ShapeNet360 \cite{dourado2020semantic}, which takes the estimated depth  map and the original 360$^{\circ}$ image as inputs. After mapping the predicted material labels into the 3D scene, the Unity virtual platform \cite{Unity} renders the immersive sound with the Steam Audio plug-in \cite{steam}. They show that this single-shot method achieves comparable performance compared with stereo-based methods \cite{mona2022audio}, partially owing to our material segmentation network, the DBAT.


\subimport{../tikzfiles/}{3dwithmaterial.tex}

% \subimport{../tikzfiles/}{edt.tex}

% \subimport{../tikzfiles/}{rt60.tex}

==> modules/tables/netdissec_table_lmd.tex <==
\begin{table*}
    \centering
    \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
    \hline
       ~ & ResNet-152 & ResNest-101 & EfficientNet-b5 & Swin-t & CAM-SegNet-DBA & DBAT \\ \hline
        Pixel Acc (LMD) & 80.68 & 82.45 & 83.17 & 84.7 & 86.12 & 86.85 \\ \hline
        $|\text{Count}|$ & 1197 & 929 & 129 & 304 & 480 & 490 \\ \hline
        Count\% & 58.45 & 45.36  & 25.20 & 39.58  & 62.50 & 63.80  \\ \hline
        $|\text{Color}|$ & 2 & 1 & 0 & 0 & 0 & 0 \\ \hline
        Color\% & 0.10 & 0.05 & 0 & 0 & 0 & 0 \\ \hline
        $|\text{Texture}|$ & 217 & 210 & 0 & 172 & 251 & 282 \\ \hline
        Texture\% & 10.60 & 10.25  & 0 & 22.40 & 32.68  & 36.72 \\ \hline
        $|\text{Part}|$ & 321 & 189 & 37 & 12 & 23 & 28 \\ \hline
        Part\% & 15.67  & 9.23 & 7.23 & 1.56 & 2.99  & 3.65 \\ \hline
        $|\text{Object}|$ & 630 & 405 & 88 & 94 & 151 & 120 \\ \hline
        Object\% & 30.76  & 19.78 & 17.19 & 12.24 & 19.66  & 15.63 \\ \hline
        $|\text{Scene}|$ & 9 & 41 & 3 & 18 & 35 & 50 \\ \hline
        Scene\% & 0.44 & 2.00  & 0.59 & 2.34  & 4.56 & 6.51  \\ \hline
        Neuron Count & 2048 & 2048 & 512 & 768 & 768 & 768 \\ \hline
    \end{tabular}
    \label{net_dissec_raw_content}
    \caption{The raw content of the disentangled neurons for each network, evaluated on the LMD, including the raw number and its corresponding percentage aligned to each semantic concepts.}
\end{table*}

==> tikzfiles/3dwithmaterial.tex <==
\begin{figure}
\centering
\noindent\resizebox{1\columnwidth}{!}{



\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,366); %set diagram left start at 0, and has height of 366

%Image [id:dp000050779429938918597] 
\draw (343.95,121.3) node  {\includegraphics[width=927pt,height=920pt]{images/application/SystemOverview.PNG}};


\end{tikzpicture}

}
\caption{End-to-end system structure: a single 360$^{\circ}$ image input to estimate monocular depth. Both materials recognition and 3D model reconstruction are processed in parallel. Results are integrated into Unity for complete 3D scene with materials labels to estimate and evaluate the acoustics environment. }
\label{3d_scenes_mat}
\end{figure}

==> tikzfiles/edt.tex <==
\begin{figure}
\centering
\noindent\resizebox{1\columnwidth}{!}{



\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,366); %set diagram left start at 0, and has height of 366

%Image [id:dp000050779429938918597] 
\draw (343.95,121.3) node  {\includegraphics[width=573pt,height=426pt]{images/application/EDT.PNG}};


\end{tikzpicture}

}
\caption{The EDTs reported on four scenes. }
\label{3d_edt}
\end{figure}

==> tikzfiles/netdissec_coorelation_lmd.tex <==
\begin{figure*}
\centering
\noindent\resizebox{2\columnwidth}{!}{



\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,366); %set diagram left start at 0, and has height of 366

%Image [id:dp000050779429938918597] 
\draw (343.95,121.3) node  {\includegraphics[width=373.42pt,height=102.45pt]{moreimgs/plot_coorelation.png}};


\end{tikzpicture}

}
\caption{The correlation coefficients of each semantic concepts (measured with absolute count and percentage) against accuracy evaluated on the LMD. }
\label{netdissec-lmd_correlation}
\end{figure*}

==> tikzfiles/rt60.tex <==
\begin{figure}
\centering
\noindent\resizebox{1\columnwidth}{!}{



\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,366); %set diagram left start at 0, and has height of 366

%Image [id:dp000050779429938918597] 
\draw (343.95,121.3) node  {\includegraphics[width=559pt,height=421pt]{images/application/RT60.PNG}};


\end{tikzpicture}

}
\caption{The RT60s reported on four scenes. }
\label{3d_rt60}
\end{figure}
